Enhancing Foundation Models for Time Series Forecasting via Wavelet-based Tokenization

How to best develop foundational models for time series forecasting remains an important open question. Tokenization is a crucial consideration in this effort: what is an effective discrete vocabulary for a real-valued sequential input? To address this question, we develop WaveToken, a wavelet-based tokenizer that allows models to learn complex representations directly in the space of time-localized frequencies. Our method first scales and decomposes the input time series, then thresholds and quantizes the wavelet coefficients, and finally pre-trains an autoregressive model to forecast coefficients for the forecast horizon. By decomposing coarse and fine structures in the inputs, wavelets provide an eloquent and compact language for time series forecasting that simplifies learning. Empirical results on a comprehensive benchmark, including 42 datasets for both in-domain and zero-shot settings, show that WaveToken: i) provides better accuracy than recently proposed foundation models for forecasting while using a much smaller vocabulary (1024 tokens), and performs on par or better than modern deep learning models trained specifically on each dataset; and ii) exhibits superior generalization capabilities, achieving the best average rank across all datasets for three complementary metrics. In addition, we show that our method can easily capture complex temporal patterns of practical relevance that are challenging for other recent pre-trained models, including trends, sparse spikes, and non-stationary time series with varying frequencies evolving over time.

==> sections/warmup.tex <==
\section{A brief tour of wavelets}\label{sec:warmup}

\subsection{Motivation: From the fourier transform to the wavelet transform}
\label{sec:ft_to_wt}

The Fourier Transform (FT) allows one to map a signal from the time domain to the frequency domain by computing the signal's projection onto a basis of complex exponentials, which represent sine and cosine functions of varying frequencies. 
This process effectively decomposes the signal into its constituent frequency components. 
The main drawback of the Fourier Transform is that, while having high resolution in the frequency domain, it has zero resolution in the time domain. 
In other words, it cannot tell at which location in time these frequencies occur in the original signal. 
The Short-Time Fourier Transform (STFT) tries to overcome this issue by splitting the original signal in different windows and applying the Fourier Transform in each of them. 
Nonetheless, the fixed window immediately implies a trade-off: the smaller the size of the window, the higher the resolution in time domain, the lower the resolution in frequency domain, and vice versa. 
This is widely known as the Uncertainty Principle \citep{oppenheim2010discrete}.

The Wavelet Transform (WT) addresses this limitation by employing a quickly decaying zero-mean oscillatory function, known as the mother wavelet, which inherently adapts its time-frequency resolution to the signal's characteristics. By dilating or compressing the wavelet, its time support varies inversely with its frequency, thus providing high time resolution for high-frequency components and high frequency resolution for low-frequency components. 
This dual localization property, achieved through the modulation of the wavelet's scale parameter, enables the WT to efficiently analyze non-stationary signals whose spectral content evolves over time, a phenomenon often referred to as \textit{time-frequency localization} \citep{daubechies1992ten, mallat2009wavelet}.


\subsection{The haar wavelet and the discrete wavelet transform}\label{sec:haar_dwt}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\textwidth]{figures/schema.png}
    \caption{\textbf{High-level depiction of our method.} \textit{(Left)} \wavetoken{}
    first re-scales the input time series by computing $\tilde{x}_t = (x_t - \mu_{1:C})/\sigma_{1:C}$, then it applies the DWT and possibly thresholds the resulting detail coefficients to zero (red crosses). The wavelet coefficients are finally quantized to bins of optimal size given their empirical distribution, and then concatenated together (excluding the first $J-1$ approximations). \textit{(Right)} 
    After pretraining on a large corpus of time series, at inference time the model 
    %\michael{See my coments at the end of the intro, maybe point out this can be any model, but we apply it to Chronos.}\luca{See my comment below}
    samples autoregressively from the categorical output distribution and yields coefficients at all decomposition levels, which are pushed through the inverse tokenizer to obtain a forecast.
    %\michael{Is our novelty the left, and we say we could plug it into various existing things, an example of which is on the right? If we are clear about that, then I think we can say that Chronos is the thing we plug into on the right.}\luca{We decided to detach ourselves as much as we can from Chronos at least in the text, to avoid reviewers saying “why not that framework then”.}
    }
    \label{fig:schema}
\end{figure}

Wavelet families consist of basis functions that can be divided into two primary types: the scaling function (often referred to as the ``father'' wavelet), which captures the low-frequency, coarse structure of the signal (the \textit{approximation}), and the wavelet function (often referred to as the ``mother'' wavelet), which captures the high-frequency components (the \textit{detail}) of the signal. 
The ``father'' and ``mother'' wavelets give rise to ``son'' and ``daughter'' wavelets through scaling and translation. 
Here, we briefly formalize these concepts in the context of the Haar wavelet \citep{haar1911theorie}, a simple yet pedagogically significant wavelet family. 
For an extensive introduction to wavelets and their applications, see, for example, \citet{mallat2009wavelet}, \citet{daubechies1992ten} and \citet{strang1996wavelets}.

The Haar father wavelet is given by $\phi(x) = \mathbb{I}(x \in [0, 1])$. The corresponding son wavelet is
\begin{equation*}\label{eq:haar_son}
     \phi_{k, j}(x) = 2^{j/2}\phi(2^j x-k) = 
     \begin{cases} 2^{j/2}, &\text{if } \frac{k}{2^j} \leq x \leq \frac{k+1}{2^j} \\ 0, &\text{otherwise},
     \end{cases}
\end{equation*}
where $k,j \in \mathbb{N}$. Note that $\phi_{k, 0}(x)$ generates an orthonormal basis for functions with jumps at the integers, whose space we denote by $V_0$. The dilations and translations $\phi_{k, j}(x)$ span orthonormal spaces $V_j$ for functions with jumps at $k/2^j$, and satisfy $V_{j+1} \supset V_j \supset \cdots \supset V_0$. With these bases, we can represent an arbitrary function $f(x)$ in $V_{j+1}$ by taking a component in $V_j$ (the \textit{approximation}) plus the orthogonal complement of $V_j$ to $V_{j+1}$, which we denote by $W_j$ (the \textit{detail}). In other words, we represent $f$ in $V_{j+1}$ by taking its orthogonal decomposition $V_{j+1} = V_j \oplus W_j$. The space $W_0$ is spanned by the mother wavelet
\begin{equation*}\label{eq:haar_mother}
    \psi(x) = \phi(2x) - \phi(2x-1) = 
    \begin{cases} 1, &\text{if } 0 \leq x < \frac{1}{2} \\ -1, &\text{if }\frac{1}{2} \leq x \leq 1 \\ 0, &\text{otherwise}
    \end{cases},
\end{equation*}
whose dilations and translations $\psi_{k, j} = 2^{j/2}\psi(2^j x-k)$ form an orthonormal basis for each $W_j$. Putting this all together, we can represent a function at different resolution levels by breaking down the level-$j$ approximation component $V_j$ to level-$(j-1)$ detail and approximation components, and so on: $V_J = V_J \oplus W_J = V_0 \oplus W_0 \oplus W_1 \cdots W_{J-1}$. A wavelet decomposition is then a linear combination of elements in these subspaces:
\begin{equation*}\label{eq:wavedec}
    f(x) = \sum_{k=-\infty}^{\infty}a_k\phi_{k, J}(x) + \sum_{j=1}^J\sum_{k=-\infty}^{\infty} d_{k, j}\psi_{k, j}(x),
\end{equation*}
where only a finite number of coefficients $a_k$ and $d_{k, j}$ are non-zero. 

How do we compute $a_k$ and $d_{k, j}$ in practice? The multi-resolution theory of \citet{mallat1989multiresolution} and \citet{meyer1992wavelets} offers an elegant and efficient solution: any wavelet that generates an orthonormal basis can be characterized by a conjugate mirror filter. The mapping from a discretized signal to a sequence of wavelet coefficients is then implemented as a filter bank made of a cascade of high-pass and low-pass filters associated with the mother and father wavelets, and is called Discrete Wavelet Transform (DWT)\footnote{We always refer to the \textit{decimated} DWT. For a comparison with the \textit{undecimated} DWT, see \citet{mallat2009wavelet}.}. For the Haar family, the approximation components are associated with averaging filters (low-pass), while the detail components are associated with distance filters (high-pass). The DWT convolves these filters with the signal and then downsamples by a factor of two to eliminate the repeated information. The result is an  array of detail coefficients $\{d_k\}_j$ and approximation coefficients $\{a_k\}_j$. The latter can be further decomposed into new approximation and detail coefficients at the next level and the process can continue recursively, resulting in a hierarchical and multi-resolution decomposition of the signal. Figure~\ref{fig:wave_fam_dec} (right) shows this for a particular time series.

The DWT has a computational complexity of $\mathcal{O}(N)$, with $N$ being the length of the input signal. This is due to \textit{i)} the filtering operation requiring a constant amount of work proportional to the signal length, and \textit{ii)} the down-sampling operation halving the signal at each of the $\log_2 N$ levels: this leads to a total amount of work equal to $N(1 + \frac{1}{2} + \frac{1}{4} + \cdots)$, which converges to $2N$. Note that this is even faster than the FFT algorithm, which has a computational complexity of $\mathcal{O}(N\log N)$.

==> style_files/custom_stuff.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% additional packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{makecell}
\usepackage{xspace}
% This changes the font for monospaced text (\texttt) to a visually pleasing one
\usepackage{inconsolata}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% custom commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\wavetoken}{\texttt{WaveToken}\xspace}
\newcommand{\wavetokenmini}{\texttt{WaveToken-Mini}\xspace}
\newcommand{\wavetokensmall}{\texttt{WaveToken-Small}\xspace}
\newcommand{\wavetokenbase}{\texttt{WaveToken-Base}\xspace}
\newcommand{\wavetokenlarge}{\texttt{WaveToken-Large}\xspace}
\DeclareRobustCommand{\bftable}{\begingroup\bfseries\aftergroup\endgroup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% algos
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\codecomment}[1]{\textbf{\color{black}// #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% meta (todo & comments)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\TODO}[1]{\textcolor{orange}{TODO:~{#1}}}
\newcommand{\QUESTION}[1]{\textcolor{red}{QUESTION:~{#1}}}
\newcommand{\NOTE}[1]{\textcolor{violet}{NOTE:~{#1}}}

% Uncomment the following line to hide all comments
\newcommand{\nocomments}{}

\ifdefined\nocomments
    \newcommand{\luca}[1]{}
    \newcommand{\fatir}[1]{}
    \newcommand{\boran}[1]{}
    \newcommand{\xiyuan}[1]{}
    \newcommand{\andrew}[1]{}
    \newcommand{\michael}[1]{}
    \newcommand{\christos}[1]{}
    \newcommand{\youngsuk}[1]{}
    \newcommand{\syama}[1]{}
    \newcommand{\danielle}[1]{}
    \newcommand{\bernie}[1]{}
\else
    \newcommand{\luca}[1]{\textbf{\color{olive}[Luca: #1]}}
    \newcommand{\fatir}[1]{\textbf{\color{teal}[Fatir: #1]}}
    \newcommand{\boran}[1]{\textbf{\color{purple}[Boran: #1]}}
    \newcommand{\xiyuan}[1]{\textbf{\color{cyan}[Xiyuan: #1]}}
    \newcommand{\andrew}[1]{\textbf{\color{brown}[Andrew: #1]}}
    \newcommand{\michael}[1]{\textbf{\color{blue}[Michael: #1]}}
    \newcommand{\christos}[1]{\textbf{\color{lime}[Christos: #1]}}
    % do not use \small because it applies it to the whole text
    \newcommand{\youngsuk}[1]{{\color{green}[YP: #1]}}
    \newcommand{\syama}[1]{\textbf{\color{orange}[Syama: #1]}}
    \newcommand{\danielle}[1]{\textbf{\color{green}[Danielle: #1]}}
    \newcommand{\bernie}[1]{\textbf{\color{yellow}[Bernie: #1]}}

    \newcommand{\xxcomment}[4]{\textcolor{#1}{[$^{\textsc{#2}}_{\textsc{#3}}$ #4]}}
    \newcommand{\agw}[1]{\xxcomment{red}{A}{W}{#1}}
\fi

